Open Domain Web Keyphrase Extraction Beyond Language Modeling

This paper studies keyphrase extraction in real-world scenarios where documents are from diverse domains and have variant content quality. We curate and release OpenKP, a large scale open domain keyphrase extraction dataset with near one hundred thousand web documents and expert keyphrase annotations. To handle the variations of domain and content quality, we develop BLING-KPE, a neural keyphrase extraction model that goes beyond language understanding using visual presentations of documents and weak supervision from search queries. Experimental results on OpenKP confirm the effectiveness of BLING-KPE and the contributions of its neural architecture, visual features, and search log weak supervision. Zero-shot evaluations on DUC-2001 demonstrate the improved generalization ability of learning from the open domain data compared to a specific domain.

==> Todo.tex <==
\section{TODO}

Next Week:

Chuan Hu: Run baselines on our data.
Approximate order:
\begin{enumerate}
\item seq2seq + Copy (CopyRNN): https://github.com/memray/seq2seq-keyphrase-pytorch  (High priority)
\item TF-IDF: In house
\item Text Rank: https://github.com/summanlp/textrank or https://github.com/boudinfl/pke
\item Single Rank: https://github.com/boudinfl/pke
\item TopicRank: https://github.com/boudinfl/pke
\item Feature-based supervised method: In House
\end{enumerate}

Testing our models on this public data set: DUC 2001: https://github.com/boudinfl/duc-2001-pre. No need to train on this one, just test our web-page trained model. TF-iDF, TextRank, SingleRank, ExpandRank, CopyRNN scores can borrow from Table 6 of https://arxiv.org/pdf/1808.07185.pdf. Need to get our method and our feature-based baseline scores on this one.


Lee Xiong: Get overall evaluation numbers on both automatic evaluation and human evaluation, do ablation studies
\begin{enumerate}
\item All overall results and compared with baselines on our dataset
\item Ablation Studies as listed in the experiments section.
\end{enumerate}

Lee Xiong: analyses on our annotation dataset.


Chenyan: Coordinate the experiment process and paper writing.





==> archive/agreement.tex <==


% , tasks with judgment overlap to spot differences in guideline interpretation and evaluation of these overlap tasks to understand human level baselines. To set a human baseline, we took a sub sample of 55 URLs selected at random and had 5 separate judges provide annotations. To measure agreement we looked at both keyphrase exact match and unigram overlap and employed various methods to select an answer as the ground truth. 
% \begin{itemize}
%     \item \textit{Highest Agreement} For each URL, each expert annotation is compared to their peers and we select the annotation with highest agreement as truth.
%     \item \textit{Pairwise:} For each URL, each expert annotation is compared to all other annotations.
% \end{itemize}
% As shown in table \ref{tab:agreements}, agreement between judges is high independent of evaluation metric. Our experts were not immune to mistakes and in studying judgment disagreement we found the disagreement was mostly chunking and keyphrase selection. 

Chunking disagreement is the biggest source of annotator variance and perhaps the easiest to understand. Judges may agree on the salience of concepts but choose different text chunks to represent the concepts, for example ``President Barack Obama" vs. ``Barack Obama'' . Take the example document https://quizlet.com/8136549/rnaprotein-synthesis-flash-cards/ which is a website that is a study page for rna and protien \ao{protein}. Some judges selected the term 'Protein Synthesis' while others just did 'Protein' and other yet did 'Protein' and 'Synthesis' as separate terms. We do not believe this is a concern in the dataset because the disagreement is not on what is important, just how to chunk and separate. 

Keyphrase selection disagreement is the more common judge error which is rooted in the task. Since judges were asked to provide 1-3 keyphrases disagreement on the 3rd keyphrase is prevalent. If we focus on agreement of the first keyphrase the EM agreement jumps up to 69\%. If we observe one sample judgement on a tax webpage, 4 out of 5 judges choose [Roth IRAs, tax-free income, federal-tax rules] the final judge   looking at a document like http://endgeoengineering.com/geoengineering.html where judges  had perfect agreement on 'geoengineering' but disagree around secondary keyphrases such as 'chemtrails' vs 'Earths's atmosphere'. 
We manually looked at every instance of judge overlap to understand the distributiuon of disagreement. This disagreement actually is beneficial because it provides a broader spectrum from where to draw possible keyphrases. We manually inspected each instance of agreement and found that for keyphrase selection, there is disgreement for all URLS with at least one judge. For one such document, relating to taxes, 4 judges had exactly the same answer for all 3  [[{'IRAs', 'Roth'}, {'income', 'tax-free'}, {'federal', 'rules', 'tax'}],
  [{'IRAs', 'Roth'}, {'income', 'tax-free'}, {'federal', 'rules', 'tax'}],
  [{'IRAs', 'Roth'}, {'income', 'tax-free'}, {'federal', 'rules', 'tax'}],
  [{'IRAs', 'Roth'}, {'Kiplinger'}]


==> archive/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

%Open Domain KPE
% a new dataset to be released.

%BLING model, convolutional transformer, visual features, and weak supervision

%Best accuracy.
%Contribution of each components

%Generalize well


%future work

    %benchmark
        %more labels
        %pair with other tasks
        %to facilitate future research in
                %deeper models
                %connect it with downstream tasks
    
This paper studies keyphrase extraction in the real-world scenario: documents with domains and varying content quality.
To overcome the scarcity of diverse training data, we curate and release OpenKP, the first large scale keyphrase extraction benchmark with real-world web pages and expert keyphrase annotations.
Using this dataset, we then develop BLING-KPE, a keyphrase extraction system that employs a convolutional transformer architecture, leverages visual features, and builds on weak supervisions from search logs. These diverse data sources and training regime produce a powerful model that generalizes to varied domains and goes beyond content modeling.

Our experiments on OpenKP and our auxiliary Query Prediction task demonstrate the strong performance of BLING-KPE. In our ablation study, the effects of BLING-KPE's network architecture, visual features and search-based weak supervision, as well as their different characteristics showcase how the model joins diverse methods to deliver powerful performance. BLING-KPE delivers robust improvements across all metrics and tasks when compared to previous approaches and our own highly optimized production system across all metrics and tasks.


By learning from open domain real-world data makes BLING-KPE is able to generalize to data scarce domains without needing any domain specific training data. This generalizable performance is shown by being the only neural keyphrase method that outperforms traditional KPE methods when evaluated in the zero-shot scenario on DUC-2001 where previous neural keyphrase approaches have not been able to handle the domain differences from their training data (scientific papers) and DUC-2001's news articles. 


Our future work plans to extend OpenKP benchmark with more expert labels, increase the diversity of document domains, and increase the size, potentially to 150K web pages, with refined annotation guidelines to further improve the annotation quality. It will facilitate the exploration of deeper neural architectures in future research.
We also plan to connect OpenKP with other downstream applications in our benchmark, to promote more future studies in utilizing the better document understanding from keyphrases in down-stream applications.







    





==> table/tablebackup.tex <==
\begin{table*}[h]
    \centering
     \caption{Keyphrase Extraction Accuracy. Relative performances in percentages are compared to \texttt{Production}, the production KPE system. $\dagger, \ddagger, \mathsection, \mathparagraph$ mark the statistically significant improvements over \texttt{TFIDF}$^\dagger$, \texttt{LeToR}$^\ddagger, \texttt{Production}$^\mathsection, \texttt{CopyRNN}$^\mathparagraph$. 
    \label{tab:overal}}
    \small
    \begin{tabular}{l|cccccc|cccccc} \hline \hline
    & \multicolumn{6}{c|}{\textbf{OpenKP}} 
    & \multicolumn{6}{c}{\textbf{Query Prediction}} \\ \hline  
    % \textbf{Method}     
    % &  \multicolumn{2}{c}{\textbf{Precision@1}} &  \multicolumn{2}{c}{\textbf{Precision@3}}  &  \multicolumn{2}{c|}{\textbf{Recall@5}}
    %   &  \multicolumn{2}{c}{\textbf{Precision@1}} &  \multicolumn{2}{c}{\textbf{Precision@3}}  &  \multicolumn{2}{c}{\textbf{Recall@5}}
    % \\ \hline
           \textbf{Method}     
    &  \textbf{P@1} &  \textbf{R@1}
     &  \textbf{P@3} &  \textbf{R@3}
      &  \textbf{P@5} &  \textbf{R@5} 
      &  \textbf{P@1} &  \textbf{R@1}
     &  \textbf{P@3} &  \textbf{R@3}
      &  \textbf{P@5} &  \textbf{R@5} 
    \\ \hline
{TFIDF} 
& 0.2760708 & 0.14513 & 0.18 & 0.2779 & 0.13525 & 0.34197  & 0.311518 & 0.25665 & 0.163 & 0.3888 & 0.10728 & 0.42171
\\ 
{TextRank} 
& 0.0795662 & 0.04162 & 0.061 & 0.0948 & 0.05405 & 0.13739 & 0.1080554 & 0.09 & 0.075 & 0.1814 & 0.06154 & 0.24614 \\ 
{LeToR} 
& 0.3023097 & 0.15879 & 0.171 & 0.2647 & 0.12564 & 0.32078 & 0.2774181 & 0.22963 & 0.144 & 0.3456 & 0.10125 & 0.40118 \\ \hline
{Production}
& 0.351822 & 0.18622 & 0.191 & 0.2941 & 0.12964 & 0.32803 & 0.333 & 0.274 & 0.175 & 0.42 & 0.115 & 0.456 \\ 
{Production (Body)}
& 0.2067834 & 0.10685 & 0.126 & 0.1913 & 0.09163 & 0.22739 & 0.3162384 & 0.25901 & 0.172 & 0.4115 & 0.11291 & 0.44655 \\
\hline
{CopyRNN}
&  &  &  &  & &  & & & & \\ \hline
{BLING-KPE}& 0.4022232 & 0.21918 & 0.254 & 0.3941 & 0.19513 & 0.48925 & 0.5404789 & 0.44987 & 0.305 & 0.6594 & 0.21441 & 0.73681 \\ \hline \hline
    \end{tabular}
   
\end{table*}


\begin{table*}[h]
    \centering
     \caption{Model Ablations. Relative performances in percentages and statistically significant differences$^*$ are compared to \texttt{Full Model}.
     \texttt{No Location} drops both the position embedding.
    \label{tab:ablation}}
    \small
    \begin{tabular}{l|cccccc|cccccc} \hline \hline
    & \multicolumn{6}{c|}{\textbf{OpenKP}} 
    & \multicolumn{6}{c}{\textbf{Query Prediction}} \\ \hline  
    % \textbf{Method}     
    % &  \multicolumn{2}{c}{\textbf{Precision@1}} &  \multicolumn{2}{c}{\textbf{Precision@3}}  &  \multicolumn{2}{c|}{\textbf{Recall@5}}
    %   &  \multicolumn{2}{c}{\textbf{Precision@1}} &  \multicolumn{2}{c}{\textbf{Precision@3}}  &  \multicolumn{2}{c}{\textbf{Recall@5}}
    % \\ \hline
       \textbf{Method}     
    &  \textbf{P@1} &  \textbf{R@1}
     &  \textbf{P@3} &  \textbf{R@3}
      &  \textbf{P@5} &  \textbf{R@5} 
      &  \textbf{P@1} &  \textbf{R@1}
     &  \textbf{P@3} &  \textbf{R@3}
      &  \textbf{P@5} &  \textbf{R@5} 
    \\ \hline
{No Transformer} 
& 0.3890653 & 0.2109 & 0.252 & 0.3882 & 0.19531 & 0.48711 & 0.4898162 & 0.40808 & 0.274 & 0.6209 & 0.19461 & 0.70292 \\
{No Position} 
& 0.3943587 & 0.21356  & 0.254 & 0.3911 &  0.1958 & 0.48488 & 0.5438499 & 0.45253 & 0.312 & 0.6716  & 0.21928 & 0.75016 \\ \hline
{No Visual} 
& 0.3697822 & 0.20151  & 0.238 & 0.3684 & 0.1841 & 0.45959  & 0.4876398 & 0.40592 & 0.281 & 0.6119  & 0.20037 & 0.6933 \\    
{No Font} 
& 0.3663793 & 0.19984  & 0.237 & 0.3667 & 0.18258 & 0.45521  & 0.498090874 & 0.41492354 & 0.286947 & 0.6233424  & 0.20400807 & 0.70513473 \\    
{No Size\&Location} 
& 0.4032819 & 0.21833  & 0.255 & 0.3934 & 0.19651 & 0.48829  & 0.52117493 & 0.43397298 & 0.299611 & 0.6491277  & 0.2116293 & 0.72847706 \\ 
{No DOM Structure} 
& 0.3934513 & 0.21383  & 0.248 & 0.3829 & 0.19052 & 0.47377  & 0.52502591 & 0.43764941 & 0.298704 & 0.6447337  & 0.21055037 & 0.72310206 \\  \hline
{No Query Prediction} 
& 0.3724289 & 0.20119  & 0.243 & 0.3749 & 0.18783 & 0.47048  
& n.a. & n.a. & n.a. & n.a. & n.a. & n.a.
\\ \hline
{Full Model}
& 0.4022232 & 0.21918 & 0.254 & 0.3941 & 0.19513 & 0.48925 & 0.5404789 & 0.44987 & 0.305 & 0.6594 & 0.21441 & 0.73681 \\ 
\hline \hline
\end{tabular}
\end{table*}
